Sequential Solutions in Machine Scheduling Games

We consider the classical machine scheduling, where $n$ jobs need to be scheduled on $m$ machines, and where job $j$ scheduled on machine $i$ contributes $p_{i,j}\in \mathbb{R}$ to the load of machine $i$, with the goal of minimizing the makespan, i.e., the maximum load of any machine in the schedule. We study inefficiency of schedules that are obtained when jobs arrive sequentially one by one, and the jobs choose themselves the machine on which they will be scheduled, aiming at being scheduled on a machine with small load. We measure the inefficiency of a schedule as the ratio of the makespan obtained in the worst-case equilibrium schedule, and of the optimum makespan. This ratio is known as the \emph{sequential price of anarchy}. We also introduce two alternative inefficiency measures, which allow for a favorable choice of the order in which the jobs make their decisions. As our first result, we disprove the conjecture of Hassin and Yovel claiming that the sequential price of anarchy for $m=2$ machines is at most 3. We show that the sequential price of anarchy grows at least linearly with the number $n$ of players, i.e., we show that $SPoA = \Omega(n)$. Furthermore, we show that there exists an order of the jobs, resulting in makespan that is at most linearly larger than the optimum makespan. To the end, we show that if an authority can change the order of the jobs adaptively to the decisions made by the jobs so far (but cannot influence the decisions of the jobs), then there exists an adaptive ordering in which the jobs end up in an optimum schedule.

==> machine scheduling/claim-proof.tex <==
	\begin{proof}[of Claim]
	Consider the best alternative solution $\copt'_h$, that is, the best allocation for the remaining jobs $R_h$, given the allocation $A_h$ of jobs in $S_h$, such that at least one job in $R_h$ is not allocated as in $\copt_h$. 
	%We assume that all players break ties in some fixed manner and, in particular, they all prefer $\copt_h$ over $\copt'_h$ whenever their cost is the same.  
	Observe the following: 
	\begin{itemize}
		%\item The makespan of $\copt'_h$  is at least the makespan of $\copt_h$, by definition of $\copt_h$.
		\item There must be a job $J'\in R_h$ which $\copt'_h$ allocates differently from $\copt_h$ and in $\copt'_h$ this job is on a machine determining the makespan of $\copt'_h$. 
		%\item Suppose we allocate this job $J'$ as in $\copt'_h$, thus obtaining an allocation $A'_h$ for jobs $S_h \cup \{J'\}$, and remaining jobs to allocate $R'_h = R_h \setminus \{J'\}$.
%		\item The machine which determines the makespan of $\copt'_h$ must contain at least one job $J^*(h)$ which solution $\copt_h$ allocates to the other machine.
		
		
%		\item If $J'$ deviates from the constrained optimum $\copt_h$, then $\copt'_h$ is the new constrained optimum: $J'$ is allocated as in $\copt'_h$, the other previously allocated jobs are as in $A(h)$. \label{itm:claim-copt}
	\end{itemize}
	This means that if $J'$ deviates from $\copt_h$, then she is choosing the machine according to $\copt'_h$. Consider the resulting constraints $A'_h$ and $R'_h$, where we extend $A_h$ by allocating $J'$ as in $\copt'_h$ (therefore the remaining players are $R'_h=R_h \setminus \{J'\}$). Since $\copt'_h$ is the best solution among all solutions in which at least one job from $R_h$ is not allocated as in $\copt_h$, then $\copt'_h$ is a constrained optimum for such $A'_h$ and $R'_h$.  The cost of $J'$ in solution $\copt'_h$ is the corresponding makespan, which cannot be smaller than the makespan of $\copt_h$.  We can thus choose $J^*(h)=J'$ and observe that  deviating from $\copt_h$ makes $J^*(h)$ incur at least the same cost as in $\copt_h$. \qed
\end{proof}
